How Unique is Your .onion? An Analysis of the Fingerprintability of Tor Onion Services

Recent studies have shown that Tor onion (hidden) service websites are particularly vulnerable to website fingerprinting attacks due to their limited number and sensitive nature. In this work we present a multi-level feature analysis of onion site fingerprintability, considering three state-of-the-art website fingerprinting methods and 482 Tor onion services, making this the largest analysis of this kind completed on onion services to date. Prior studies typically report average performance results for a given website fingerprinting method or countermeasure. We investigate which sites are more or less vulnerable to fingerprinting and which features make them so. We find that there is a high variability in the rate at which sites are classified (and misclassified) by these attacks, implying that average performance figures may not be informative of the risks that website fingerprinting attacks pose to particular sites. We analyze the features exploited by the different website fingerprinting methods and discuss what makes onion service sites more or less easily identifiable, both in terms of their traffic traces as well as their webpage design. We study misclassifications to understand how onion service sites can be redesigned to be less vulnerable to website fingerprinting attacks. Our results also inform the design of website fingerprinting countermeasures and their evaluation considering disparate impact across sites.

==> sections/abstract.tex <==
\begin{abstract}
Recent studies have shown that Tor onion (hidden) service websites are particularly vulnerable to \wf attacks due to their limited number and sensitive nature. In this work we present a multi-level feature analysis of onion site fingerprintability, considering three state-of-the-art \wf methods and 482 Tor \hses, making this the largest analysis of this kind completed on \hses to date.  

Prior studies typically report average performance results for a given \wf method or countermeasure. We investigate which sites are more or less vulnerable to fingerprinting and which features make them so. We find that there is a high variability in the frequency at which sites are classified (and misclassified) by these attacks, implying that average performance may not be informative of the risks of particular sites.

We use a number of methods to analyze the features exploited by the different \wf methods and discuss what makes \hs sites more or less easily identifiable, both in terms of their traffic traces as well as their webpage design. We study misclassifications to understand how \hses sites can be redesigned to be less vulnerable to \wf attacks. Our results also inform the design of \wf countermeasures and their evaluation considering likely disparate impact across sites.

\end{abstract}


==> tikz/threat_model.tex <==
\begin{tikzpicture}

% Layers
\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers

% Guard
\node[anchor=center, yshift=0.15cm, xshift=-1.2cm, label={[below=1.3cm of guard,xshift=-0.4cm,yshift=0.5cm]{\scriptsize Entry}}] (guard) {\includegraphics[width=.05\textwidth]{img/relay.png}};

% Tor network
\node[right of=guard, xshift=0cm, label={[above=0.1cm of network]{\scriptsize Tor network}}, cloud, cloud puffs=15.7, cloud ignores aspect, minimum width=4.5cm, minimum height=2.5cm, align=center, draw] (network) at (0cm, 0cm) {};

% Anchors
\begin{pgfonlayer}{bg}
    \node[below of=guard, node distance=5pt] (guard_anchor) {{\tiny $-$}};
    \node[right of=guard_anchor, node distance=16pt] (network_anchor) {};
\end{pgfonlayer}

% Client
\node[left of=guard_anchor, node distance=2.3cm, label={[below=1.3cm of user,yshift=0.5cm]{\scriptsize Client}}] (user) {\includegraphics[width=.037\textwidth]{img/user.png}};

% Onion 1
\node[right of=guard_anchor, node distance=1.2cm, yshift=0.25cm, label={[below=1.2cm of onion1,yshift=0.3cm]{\scriptsize a.onion}}] (onion1) {\includegraphics[width=.04\textwidth]{img/tor.png}};

% Onion 2
\node[right of=guard_anchor, yshift=0.5cm, node distance=2.3cm, label={[below=1.2cm of onion2,yshift=0.3cm]{\scriptsize b.onion}}] (onion2) {\includegraphics[width=.04\textwidth]{img/tor.png}};

% Onion 3
\node[right of=guard_anchor, yshift=0.1cm, node distance=3.4cm, label={[below=1.2cm of onion3,yshift=0.6cm]{\scriptsize c.onion}}] (onion3) {\includegraphics[width=.04\textwidth]{img/tor.png}};

% Attacker
\node[anchor=center, yshift=1cm, xshift=-2.2cm] (attacker) {\includegraphics[width=.057\textwidth]{img/wfattacker.png}};
\node[anchor=center, yshift=-0.05cm, xshift=-2.2cm] (tap) {};
\node[above of=attacker, anchor=center, node distance=0.5cm] {{\scriptsize Adversary}};

% Arrows
\begin{pgfonlayer}{bg}
    \path[draw, -, line width=1.3pt] (user.east) -> (guard_anchor.center);
    \path[draw, ->] (attacker.south) -> (tap);
    %\path[draw, -] (guard_anchor.west) -> (network_anchor);
    
\end{pgfonlayer}

\end{tikzpicture}
    

